GraphVid: It Only Takes a Few Nodes to Understand a Video

We propose a concise representation of videos that encode perceptually meaningful features into graphs. With this representation, we aim to leverage the large amount of redundancies in videos and save computations. First, we construct superpixel-based graph representations of videos by considering superpixels as graph nodes and create spatial and temporal connections between adjacent superpixels. Then, we leverage Graph Convolutional Networks to process this representation and predict the desired output. As a result, we are able to train models with much fewer parameters, which translates into short training periods and a reduction in computation resource requirements. A comprehensive experimental study on the publicly available datasets Kinetics-400 and Charades shows that the proposed method is highly cost-effective and uses limited commodity hardware during training and inference. It reduces the computational requirements 10-fold while achieving results that are comparable to state-of-the-art methods. We believe that the proposed approach is a promising direction that could open the door to solving video understanding more efficiently and enable more resource limited users to thrive in this research field.

==> tables/notations.tex <==
\begin{table}[!ht]
\caption{Notations} 
\label{table:notations}
% \small
\centering
\begin{tabularx}{8.5cm}{|Sl|X|}
\hline
\textbf{Notation} & \textbf{Meaning} \\
\hline
$R_{t,i}$ & The $i^{th}$ superpixel generated for the $t^{th}$ frame. Each superpixel has the attributes $x,y$ denoting the coordinates if the superpixel's centroid, and the attribute $c$ to denote the mean color in that segmented region.\\
$E^{intra}$ & The set of edges connecting superpixels within frames.\\
$E^{inter}$ & The set of edges connecting superpixels between subsequent frames.\\
$d_{i,j}^t$ & Distance between the 
\hline
\end{tabularx}

\end{table}

==> tables/sota_comparison.tex <==
\begin{table}[!ht]
\caption{Comparison of model specifications for various architectures. We report Top-1 accuracy on Kinetics-400 and Charades.} 
\label{table:models}
\small
\centering
\begin{tabularx}{8.5cm}{Sl X X X X}
\hline
Model & K400 & Charades & FLOPs & Params ($\times 10^6$)\\
\hline
$GCN$ & - & - & - & -\\
$RGCN$ & - & - & - & -\\
\hline
\end{tabularx}
\end{table}
